An iterative multi-fidelity approach for model order reduction of multi-dimensional input parametric PDE systems

We propose a parametric sampling strategy for the reduction of large-scale PDE systems with multidimensional input parametric spaces by leveraging models of different fidelity. The design of this methodology allows a user to adaptively sample points ad hoc from a discrete training set with no prior requirement of error estimators. It is achieved by exploiting low-fidelity models throughout the parametric space to sample points using an efficient sampling strategy, and at the sampled parametric points, high-fidelity models are evaluated to recover the reduced basis functions. The low-fidelity models are then adapted with the reduced order models ( ROMs) built by projection onto the subspace spanned by the recovered basis functions. The process continues until the low-fidelity model can represent the high-fidelity model adequately for all the parameters in the parametric space. Since the proposed methodology leverages the use of low-fidelity models to assimilate the solution database, it significantly reduces the computational cost in the offline stage. The highlight of this article is to present the construction of the initial low-fidelity model, and a sampling strategy based on the discrete empirical interpolation method (DEIM). We test this approach on a 2D steady-state heat conduction problem for two different input parameters and make a qualitative comparison with the classical greedy reduced basis method (RBM), and further test on a 9-dimensional parametric non-coercive elliptic problem and analyze the computational performance based on different tuning of greedy selection of points.

==> flowdiag.tex <==
\huge

\coordinate (a) at (0,0);
  \coordinate (b) at ($(a)+(0,-3)$);
 
   \coordinate (d) at ($(b)+(8,1.5)$);
   
  \coordinate (e) at ($(d)+(6.05,3)$);
  \coordinate (f) at ($(d)+(6.05,-3)$);

    \coordinate (g) at ($(f)+(0,-5)$);
     \coordinate (h) at ($(g)+(8,0)$);
          \coordinate (i) at ($(h)+(0,10)$);
          \coordinate (j) at ($(i)+(6,0)$);

\coordinate (qa) at ($(b)+(5,0)$);

 
 
\node[rectangle,
    draw = black,
    text = black,
    fill = darkgray!20,
    minimum width = 2cm,
    minimum height = 2cm, align = center ] (rect-plan) at (a) {Daily CBCT};
   
 
   
\node[rectangle,
    draw = black,
    text = black,
    fill = darkgray!20,
    minimum width = 2cm,
    minimum height = 2cm, align = center] (rect-cbct) at (b) {Planning CT};
 
     
\node[diamond,
    draw = black,
    text = black,
    fill = red!5, align=center, minimum width = 1cm,
    minimum height = 1cm
    ] (d-reg) at (d) {Registration};
     
\node[rectangle,
    draw = black,
    text = black,
    fill = blue!10,
    minimum width = 2cm,
    minimum height = 2cm, align = center] (rect-regct) at (e) {Registered \\CT Image};
   
\node[rectangle,
    draw = black,
    text = black,
    fill = blue!10,
    minimum width = 2cm,
    minimum height = 2cm, align = center] (rect-trpara) at (f) {Translation \\Parameters};    
   
    \node[diamond,
    draw = black,
    text = black,
    fill = red!5, align=center, minimum width = 2.5cm,
    minimum height = 3cm
    ] (d-apply) at (g) {Apply \\Translation};
   
     \node[text width=5cm](phi) at ($(e)+(6,0)$)
    {\Huge {$\phi$}};
   
       
    \node[text width=7cm](contours) at ($(b)+(6,-9)$)
    {\Huge {CT-Contours}};
   
        \node[text width=7cm](contours) at ($(a)+(11,7.5)$)
    {\Huge {CBCT Volume}};
   
     \node[text width=7cm](contours) at ($(h)+(4,5)$)
    {\Huge {Reg. CT Mask}};
   
    \node[rectangle,
    draw = black,
    text = black,
    fill = blue!10,
    minimum width = 2cm,
    minimum height = 2cm, align = center] (rect-regctmask) at (h) {Reg. CT Mask};
 
   
\node[rectangle,
    draw = black,
    text = black,
    fill = blue!10,
    minimum width = 2cm,
    minimum height = 2cm, align = center] (rect-unet) at (i) {Multimodal\\Unet Network};  
   
      \node[rectangle,
    draw = black,
    text = black,
    fill = darkgray!20,
    minimum width = 2cm,
    minimum height = 2cm, align = center] (rect-pred) at (j) {Predicted\\ CBCT Mask};
   
      \node[rectangle,
    draw = black,
    dashed,
    text = black,
    fill = gray,
    minimum width = 36cm,
    minimum height = 30cm, fill opacity = 0.1] (rect-delphase) at ($(d)+(7,-2)$) {};  
   
   
   \draw  (rect-plan.east)--($(rect-plan.east)+(1.5,0)$)--($(rect-plan.east)+(1.5,-5)$)--(rect-cbct.east);

    \draw [-{Stealth[length=3mm, width=2mm]}] ($(d-reg.west)+(-1.8,0)$)--(d-reg.west);
   
    \draw [-{Stealth[length=3mm, width=2mm]}] (d-reg.east)--($(d-reg.east)+(3.5,0)$)--(rect-regct.south);
   
    \draw [-{Stealth[length=3mm, width=2mm]}] ($(d-reg.east)+(3.5,0)$)--(rect-trpara.north);
   
    \draw [-{Stealth[length=3mm, width=2mm]}] (rect-regct)--(rect-trpara.north);
   
     \draw [-{Stealth[length=3mm, width=2mm]}] (rect-regct.east)--(phi);
   
     \draw [-{Stealth[length=3mm, width=2mm]}] (rect-trpara.south)--(d-apply.north);

    \draw [-{Stealth[length=3mm, width=2mm]}] (d-apply.east)--(rect-regctmask);
   
   
   
   \draw [-{Stealth[length=3mm, width=2mm]}] (rect-cbct.south)--($(rect-cbct.south)+(0,-7.6)$)--(d-apply.west);
   
\draw [-{Stealth[length=3mm, width=2mm]}] (rect-plan.north)--($(rect-plan.north)+(0,5)$)--($(rect-unet)+(0,11.4)$)--(rect-unet.north);

\draw [-{Stealth[length=3mm, width=2mm]}] (rect-unet.east)--(rect-pred.west);  
   
\draw [-{Stealth[length=3mm, width=2mm]}]
(rect-regctmask.north)--(rect-unet.south);
